StaticSegFormer: An Efficient High-Performance Semantic Segmentation Based on Static Structured Pruning

Structured pruning enhances the efficiency of deep neural networks (DNNs) by eliminating groups of parameters during inference. Previous methods mostly reduce computational complexity (FLOPs), while semantic segmentation performance (mIoU) slightly drops. Accordingly, recent dynamic structured pruning methods aim at reducing the performance drop, while lowering the FLOPs even more. However, on the ADE20K and Cityscapes benchmarks, our study reveals that on a GPU platform such dynamic methods exhibit a surprisingly low frame rate far below a simple static approach, while having comparable results in mIoU and FLOPs. To address this issue, we propose a static structured pruning method for attention layers, that achieves both, a lower FLOPs and a high frame rate [fps] of the SegFormer network, the latter increased by up to 34% relative on the Cityscapes dataset, while having no mIoU performance drop at all. Our so-called StaticSegFormer method is strongest for small encoders and large images.

==> mathmacros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mathematische Macros
%
% Mathematical macros for lectures and publications
%
% (c) Prof. Dr.-Ing. Tim Fingscheidt
%     IfN / TU Braunschweig, 2006-04-30
%



\ifdefined\mathmarcosdefown
    
\else

\newcommand{\mathmarcosdefown}{}
    
\newcommand{\nomathindent}{\hspace*{-10mm}}


% Mathematische Zeichen: -------------------------------------------------------
\newcommand{\entspricht}{\widehat{=}}
\newcommand{\folgerung}{\item[$\Rightarrow$]}
\newcommand{\lift}[1]{\raisebox{1.5ex}[-1.5ex]{#1}}
\newcommand{\ld}{\log_2}
\newcommand{\sign}{{\rm sign}}
\newcommand{\erfc}{{\rm erfc}}
\newcommand{\SNRSEG}{\mathrm{SNR}_{\mathrm{seg}}}
\newcommand{\SNR}{\mathrm{SNR}}
\newcommand{\ERLEu}{\mathrm{ERLE}_u}
\newcommand{\ERLEd}{\mathrm{ERLE}_d}
%\newcommand{\conv}{\ast}
\newcommand{\conv}[1][]{\ast_{_{#1}}}
\newcommand{\circconv}{\otimes}
\newcommand{\class}{\mathrm{class}}
\newcommand{\Res}[1]{{\rm Res}\{#1\}}   % Residuum
\newcommand{\E}[1]{{\mathrm{E}}\{#1\}}  % Expectation
\newcommand{\Elr}[1]{{\mathrm{E}}\left\{#1\right\}}  % Expectation
%\newcommand{\unit}[1]{{\sf #1}}
\newcommand{\OK}{\mathbf{\sqrt{}}}
\newcommand{\QUANT}[1]{{\bf Q[}#1{\bf ]}}         % Quantisierungsfunktion
\newcommand{\Dist}{{\mathfrak{D}}}
\newcommand{\WER}{\mathrm{WER}}         % WER = Word error rate
\newcommand{\WRR}{\mathrm{WRR}}         % 1-WER = Word recognition rate
\newcommand{\ACC}{\mathrm{ACC}}         % Accuracy
\newcommand{\SER}{\mathrm{SER}}         % Sentence error rate
\newcommand{\PCorr}{\mathrm{PCorr}}     % = (1-(D+S)/R) *100%, used in htk
\newcommand{\PAcc}{\mathrm{PAcc}}       % = (1-WER) *100%, used in htk
\newcommand{\WA}{\mathrm{WA}}           % Word accuracy
\newcommand{\SA}{\mathrm{SA}}           % Sentence accuracy
\newcommand{\CS}{\mathrm{CS}}           % Confidence score
\newcommand{\LOGE}{\mathrm{logE}}       % logE parameter

% SPECOM lecture:
\newcommand{\AKF}[2][]{\varphi_{#1#1}(#2)}         % Autocorrelation function (ACF)
\newcommand{\AKFsq}[2][]{\varphi^2_{#1#1}(#2)}     % ACF^2
\newcommand{\AKFvec}[1][]{\mathbf{\boldsymbol\varphi}_{#1#1}} % ACF vector
\newcommand{\AKFmat}[1][]{\mathbf{\Phi}_{#1#1}}    % ACF matrix

\newcommand{\KKF}[2][]{\varphi_{#1}(#2)}   % Crosscorrelation function (CCF)
\newcommand{\VAR}[1][]{\sigma_{#1}^2}      % Variance
\newcommand{\VAREST}[1][]{\hat{\sigma}_{#1}^2}  % geschaetzte Varianz
\newcommand{\STDDEV}[1][]{\sigma_{#1}}     % Standardabweichung
\newcommand{\PDF}[2][]{p_{#1}(#2)}         % pdf

\newcommand{\PSD}[2][]{\Phi_{#1}(#2)}      % Power spectral density (PSD)

\newcommand{\VEC}[1]{\mathbf{#1}}          % Vector
\newcommand{\VECG}[1]{\boldsymbol{#1}}     % Vector with Greek letter
\newcommand{\MAT}[1]{\mathbf{#1}}          % Matrix
\newcommand{\MATG}[1]{\boldsymbol{#1}}     % Matrix with Greek letter

\newcommand{\LTP}[1]{\overline{#1}}        % LTP variable (as opposed to LP variable)

\newcommand{\GAUSS}{{\cal N}}              % Gaussian distribution


%%%%Integrale: El Abed-----------------------------------------------------------
\newcommand{\huellenint}{\int\!\!\!\!\!\int\limits_{\!\!\!\! A}\!\!\!\!\!\!\!\! \bigcirc \:}
\newcommand{\circint}{\int\limits_C \!\!\!\!\!\!\! \bigcirc \:}
\newcommand{\flaechenint}{\int\!\!\!\int\limits_{\!\!\!\!\!\!\! A}}


% Anordnen von Indizes usw. unter einer Funktion: ------------------------------
\newcommand{\putindex}[3]{\vtop{\hbox{\hspace{#3} $#1$}
            \hbox{\raise 6mm \hbox{$\scriptscriptstyle #2$}}}}


% Gradient von x, y, allgemein: ------------------------------------------------
\newcommand{\gradx}[0]{\vtop{\hbox{\rm grad}
            \hbox{\raise 2.5mm \hbox{\rm \hspace{2mm} \footnotesize x}}}}

\newcommand{\grady}[0]{\vtop{\hbox{\rm grad}
            \hbox{\raise 2.5mm \hbox{\rm \hspace{2mm} \footnotesize y}}}}

\newcommand{\grad}[1]{\vtop{\hbox{\rm grad}
            \hbox{\raise 2.5mm \hbox{#1}}}}


% Die Menge der reellen Zahlen: ------------------------------------------------
% \newcommand{\R}{\parbox[b]{2.4ex}{{\rm I}\hspace{-0.6ex}{\bf R}}}
% \newcommand{\Rclassic}{\parbox[b]{2.3ex}{{\rm I}\hspace{-0.6ex}{\bf R}}}
\ifdefined\N
    
\else

% \newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}

\fi

\newcommand{\I}{\mathbb{I}}
% \newcommand{\N}{\mathbb{N}}

% Real- und Imaginärteil: ------------------------------------------------------
\newcommand{\real}[1]{{\rm Re}\{#1\}}
\newcommand{\imag}[1]{{\rm Im}\{#1\}}
\newcommand{\realnoarg}{{\rm Re}}
\newcommand{\imagnoarg}{{\rm Im}}

\newcommand{\comp}[1]{\underline{#1}}
\newcommand{\rect}[1]{{\rm rect}(#1)}
\newcommand{\sinc}[1]{{\rm si}(#1)}

% System T{}: ------------------------------------------------------
\newcommand{\SYSTEM}[1]{\mathfrak{T}\{#1\}}
\newcommand{\INVSYSTEM}[1]{\mathfrak{T}^{-1}\{#1\}}

% Fouriertransformation: -------------------------------------------------------
\newcommand{\invfourier}[0]{\bullet \hspace{-1.7mm} - \hspace{-1.7mm} \circ}
\newcommand{\fourier}[0]{\circ \hspace{-1.7mm} - \hspace{-1.7mm} \bullet}
%\newcommand{\FT}[1]{\mathfrak{F}\{#1\}}
\newcommand{\DTFT}[1]{{\rm DTFT}\{#1\}}
\newcommand{\DFT}[1]{{\rm DFT}\{#1\}}
\newcommand{\DCT}[1]{{\rm DCT}\{#1\}}
\newcommand{\ZT}[1]{\mathfrak{Z}\{#1\}}
\newcommand{\ZTone}[1]{\mathfrak{Z}_1\{#1\}}
\newcommand{\LT}[1]{\mathfrak{L}\{#1\}}
\newcommand{\IFT}[1]{\mathfrak{F}^{-1}\{#1\}}
\newcommand{\IDTFT}[1]{{\rm IDTFT}\{#1\}}
\newcommand{\IDFT}[1]{{\rm IDFT}\{#1\}}
\newcommand{\IDCT}[1]{{\rm IDCT}\{#1\}}
\newcommand{\IZT}[1]{\mathfrak{Z}^{-1}\{#1\}}
\newcommand{\IZTone}[1]{\mathfrak{Z}_1^{-1}\{#1\}}
\newcommand{\ILT}[1]{\mathfrak{L}^{-1}\{#1\}}
\newcommand{\minus}{\scalebox{0.75}[1.0]{$-$}}

% Neue Theoremarten: -----------------------------------------------------------
%\newtheorem{definition}{Definition}[chapter]    % report, book
\newtheorem{Adefinition}{Definition}[section]   % article => A
%\newtheorem{satz}{Satz}[chapter]
%\newtheorem{ASatz}{Satz}[section]              % Be careful! TeX capacity exc.!
%\newtheorem{beweis}[satz]{Bew.:}
%\newtheorem{Abeweis}[Asatz]{Bew.:}


% Schriftgroessen: (sinnvoll in Matrizen u.a.) ---------------------------------
\newcommand{\bSs}{\scriptstyle}
\newcommand{\bSS}{\scriptscriptstyle}


% Numerierung mittels Ziffer im Kreis: -----------------------------------------
\newcommand{\ONE}{   ${\textstyle 1}\hspace{-3.2mm} \bigcirc$ }
\newcommand{\TWO}{   ${\textstyle 2}\hspace{-3.2mm} \bigcirc$ }
\newcommand{\THREE}{ ${\textstyle 3}\hspace{-3.2mm} \bigcirc$ }


% Bezeichnung von Groessen in der Diss: Patchen der Variablen im Mathemodus: --
\newcommand{\RB}[1]{#1'}             % bipolarer, BPSK-modulierter Empfangswert

\newcommand{\HB}[2][]{\hat{#2}_{#1}}           % bipolares Hardbit
\newcommand{\HBT}[2][]{{#2}_{#1}}              % bipolares Hardbit (transmitted
\newcommand{\HBR}[2][]{\hat{#2}_{#1}}          % bipolares Hardbit (received)
%\newcommand{\HBENC}[2][]{{#2}_{#1}}           % bipolares Hardbit (Sender)
\newcommand{\HBUNI}[2][]{\bar{#2}_{#1}}        % unipolares Hardbit
\newcommand{\HV}[2][]{{\underline{\hat{#2}}_{#1}}} % Vektor bipolarer Hardbits
                                               % (Parameter) (received)
\newcommand{\HVT}[2][]{{\underline{#2}_{#1}}}  % Vektor (bipolarer) Hardbits
                                               % (Parameter) (transmitted)
\newcommand{\HVTEST}[2][]{{\underline{#2}_{#1}^{\rm (est)}}} % Vektor
                                               % geschaetzter Hardbits
\newcommand{\HVR}[2][]{{\underline{\hat{#2}}_{#1}}} % Vektor
                                                    % bipolarer Hardbits
                                               % (Parameter) (received)
%\newcommand{\HVENC}[2][]{{\bf{#2}_{#1}}}      % Vektor (bipolarer) Hardbits
                                               % (Sender)

\newcommand{\SB}[2][]{\tilde{#2}_{#1}}         % bipolares Softbit
\newcommand{\CORR}[2][]{\tilde{#2}_{#1}}       % bipolares Softbit
\newcommand{\SBUNI}[2][]{\breve{#2}_{#1}}      % unipolares Softbit
\newcommand{\SV}[2][]{{\underline{\tilde{#2}}_{#1}}} %Vektor bipolarer Softbits

\newcommand{\EST}[2][]{{#2}_{#1}^{\rm (est)}}  % geschaetzter Parameter
\newcommand{\MS}[2][]{{#2}_{#1}^{\rm (MS)}}    % MS-geschaetzter Parameter,fett
\newcommand{\VARMS}[2][]{{#2}_{#1}^{\rm (MS)}} % MS-geschaetzter Parameter
\newcommand{\MEAN}[2][]{{#2}_{#1}^{\rm (MEAN)}} % Mean-geschaetzter Par.
\newcommand{\MAP}[2][]{{#2}_{#1}^{\rm (MAP)}}  % MAP-geschaetzter Par.
\newcommand{\ML}[2][]{{#2}_{#1}^{\rm (ML)}}    % MAP-geschaetzter Par.
\newcommand{\VAROK}[2][]{{#2}_{#1}^{\rm (OK)}} % ungestoerter Parameter
%\newcommand{\MS}[2][]{{#2}_{{#1}_{\rm MS}}}   % MS-geschaetzter Parameter,fett
%\newcommand{\VARMS}[2][]{{#2}_{{#1}_{\rm MS}}} % MS-geschaetzter Parameter
%\newcommand{\MEAN}[2][]{{#2}_{{#1}_{\rm M}}}   % Mean-geschaetzter Par.
%\newcommand{\MAP}[2][]{{#2}_{{#1}_{\rm MAP}}}  % MAP-geschaetzter Par.
%\newcommand{\ML}[2][]{{#2}_{{#1}_{\rm ML}}}    % MAP-geschaetzter Par.
%\newcommand{\VAROK}[2][]{{#2}_{{#1}_{\rm OK}}} % ungestoerter Parameter
%\newcommand{\VECold}[2][]{{#2}_{#1}}             % Vektor, Parameter (allgemein)
\newcommand{\PART}[2][]{{\tilde{#2}_{#1}}}     % unquantisierter Parameter
                                               % (Transmitter)
\newcommand{\QPART}[2][]{{#2}_{#1}}            % quantisierter Parameter
                                               % (transmitted)
\newcommand{\QPARR}[2][]{{\hat{#2}_{#1}}}      % quantisierter Parameter
                                               % (received)
\newcommand{\PAREST}[2][]{{\tilde{#2}^{\rm (est)}_{#1}}}%geschaetzter Parameter
                                               % (received)

\newcommand{\VARBER}[1][]{{p^{(#1)}_e}}    % momentane, gemessene Bitfehlerrat
\newcommand{\BER}[1][]{{p_{e#1}}}          % momentane, gemessene Bitfehlerrate

\newcommand{\PROBD}[1][]{{\rm p_{#1}}}         % p( ),Wahrscheinlichkeitsdichte
\newcommand{\PROB}[0]{{\rm P}}        % P( ),   Wahrscheinlichkeit
\newcommand{\VARPROB}[0]{{\rm Prob}}  % Prob(), Wahrscheinlichkeit

%\newcommand{\QUANTINV}[1]{{\bf Q^{-1}[}#1{\bf ]}} % Inverse Qu.funktion
\newcommand{\BMINV}[1]{{\bf BM^{-1}[}#1{\bf ]}}   % Inverses Bit-Mapping
\newcommand{\BM}[1]{{\bf BM[}#1{\bf ]}}   % Inverses Bit-Mapping



\newcommand{\EV}[1]{E\{{#1}\}}                    % Erwartungswert
\newcommand{\EVEST}[1]{\hat{E}\{{#1}\}}           % geschaetzter Erwartungswert

%\newcommand{\Dist}{\tilde{D}}
\newcommand{\AKFold}[1]{R_{#1 #1}}               % Autokorrelationsfunktion
\newcommand{\AKFEST}[1]{\hat{R}_{#1 #1}}      % geschaetzter AKF-Wert
\newcommand{\ACOVF}[1]{C_{#1 #1}}             % Autocovarianzfunktion
\newcommand{\AKCOEF}[1]{\rho_{#1 #1}}         % (Auto-) Korrelationskoeffizient
\newcommand{\RHO}[0]{\rho}                    % 1. Auto-Korrelationskoeffizient
\newcommand{\AKCOEFEST}[1]{\hat{\rho}_{#1 #1}} % geschaetzter Korr.-koeffizient
\ifdefined\MW
\else
\newcommand{\MW}[1]{\eta_{#1}}                % Mittelwert
\fi
\newcommand{\MWEST}[1]{\hat{\eta}_{#1}}       % geschaetzter Mittelwert
\newcommand{\KKFold}[2]{R_{#1 #2}}               % Kreuzkorrelationsfunktion
\newcommand{\KKCOEF}[2]{\rho_{#1 #2}}         % Kreuzkorrelationskoeffizient
\newcommand{\LDSP}[1]{\Phi_{#1 #1}}           % Leistungsdichtespektrum
\newcommand{\SFM}[0]{\gamma}                  % spektrales Flachheitsmass
\newcommand{\SD}[0]{{\rm SD}}                 % spektraler Abstand

\newcommand{\VARLB}[1][]{L_{#1}}              % L-Wert ohne Bitkomb.-Bez.nung
\newcommand{\LB}[2][]{L^{(#2)}_{#1}}               % L-Wert
\newcommand{\LV}[2][]{{\underline{L}^{(#2)}_{#1}}} % Vektor L-Werte

\newcommand{\DRtheo}[0]{\Delta R}             % theoretische Redundanz
\newcommand{\DRVtheo}[0]{\Delta R_{\rm v}}    % th. verteilungsabhaengige Red.
\newcommand{\DRKtheo}[0]{\Delta R_{\rm k}}    % th. korrelationsabh"angige Red.
\newcommand{\DR}[0]{\Delta R'}                % nutzbare Redundanz
\newcommand{\DRV}[0]{\Delta R_{\rm v}'}       % nb. verteilungsabhaengige Red.
\newcommand{\DRK}[0]{\Delta R_{\rm k}'}       % nb. korrelationsabh"angige Red.
\newcommand{\RBRUTTO}[0]{R_{\rm brutto}}      % Bruttobitrate
\newcommand{\RCHCOD}[0]{R_{\rm CHCOD}}        % Nettobitrate CHCOD
\newcommand{\RSD}[0]{R_{\rm SD}}              % Nettobitrate SD
\newcommand{\DRCHCOD}[0]{\Delta R_{\rm CHCOD}} % Redundanz durch Kanalcod. (r)
\newcommand{\GPtheo}[0]{G_p}                  % theoretischer Praedikt.Gewinn
\newcommand{\GP}[0]{G_p'}                     % real erreichter Praedikt.Gewinn
\newcommand{\NGD}[0]{\epsilon}                % Nutzungsgrad der Redundanz
\newcommand{\NGV}[0]{\epsilon_{\rm v}}        % ... der verteilungsabh. Red.
\newcommand{\NGK}[0]{\epsilon_{\rm k}}        % ... korrelationsabh. Red.
\newcommand{\DRVLMQ}[0]{\Delta R_{\rm v (LMQ)}'}  % nb. vert.abh. Red. des LMQ
\newcommand{\DRVMEQ}[0]{\Delta R_{\rm v (MEQ)}'}  % nb. vert.abh. Red. des MEQ


\newcommand{\ARN}[0]{\bar{N}}                 % echte AR-Ordnung eines Par's

\newcommand{\FA}[0]{f_A}                      % Abtastfrequenz

\newcommand{\CHF}[1]{{\rm \Psi_{#1}}}         % Charakteristische Funktion


%==============================================================================
% Hier folgen Macros, die zwar nicht mathematischer Natur sind, jedoch
% in texten haeufig gebraucht werden.


% Symmetrische Zeileneinstellung fuer Tabellen (Stuetze): ---------------------
\newcommand{\stz}{\rule{0mm}{2.3ex}}
\newcommand{\stzsym}{\rule[-0.8ex]{0mm}{3.1ex}}
\newcommand{\stzdown}{\rule[-1.2ex]{0mm}{3.5ex}}
\newcommand{\stzlargesym}{\rule[-1.8ex]{0mm}{5.1ex}}

% Abkuerzung fuer die Tabulator-Umgebung: -------------------------------------
\newcommand{\btb}{     \begin{tabbing}             }
\newcommand{\bte}{     \end{tabbing}               }

% Transposed "T": ------------------------------------------------------
% \newcommand{\T}[0]{\mathsf{T}}

% Own Stuff --------------------------

\newcommand{\remHyp}[1]{\NoHyper#1\endNoHyper}

\fi

==> tables/mathematical_formulations.tex <==
\ifdefined\mathmformulationsdef
    
\else

\newcommand{\mathmformulationsdef}{}

\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\src}[0]{{\mathcal{D}^S}}
\newcommand{\tgt}[0]{{\mathcal{D}^T}}

\newcommand{\network}[1]{{\texttt{#1}}}

\newcommand{\mv}{\_\_.\_}

%DATASETS
\newcommand{\datatrain}[0]{{\mathcal{D}_\mathrm{train}}}
\newcommand{\datatrainstar}[0]{{\mathcal{D}_\mathrm{train*}}}
\newcommand{\datafull}[0]{{\mathcal{D}_\mathrm{full}}}
\newcommand{\dataval}[0]{{\mathcal{D}_\mathrm{val}}}
\newcommand{\datatest}[0]{{\mathcal{D}_\mathrm{test}}}
\newcommand{\datavalstar}[0]{{\mathcal{D}_\mathrm{val*}}}
\newcommand{\datateststar}[0]{{\mathcal{D}_\mathrm{test*}}}
\newcommand{\datadev}[0]{{\mathcal{D}_\mathrm{dev}}}
\newcommand{\dataooddev}[0]{{\mathcal{D}^\mathrm{OOD}_\mathrm{dev}}}
\newcommand{\databench}[0]{{\mathcal{D}_\mathrm{BM}}}

\newcommand{\cstrain}[0]{{\mathcal{D}^\mathrm{CS}_\mathrm{train}}}
\newcommand{\cstrainstar}[0]{{\mathcal{D}^\mathrm{CS}_\mathrm{train*}}}
\newcommand{\csval}[0]{{\mathcal{D}^\mathrm{CS}_\mathrm{val}}}
\newcommand{\cstest}[0]{{\mathcal{D}^\mathrm{CS}_\mathrm{test}}}
\newcommand{\csvalstar}[0]{{\mathcal{D}^\mathrm{CS}_\mathrm{val*}}}
\newcommand{\csteststar}[0]{{\mathcal{D}^\mathrm{CS}_\mathrm{test*}}}
\newcommand{\csdev}[0]{{\mathcal{D}^\mathrm{CS}_\mathrm{dev}}}

\newcommand{\adetrain}[0]{{\mathcal{D}^\mathrm{ADE}_\mathrm{train}}}
\newcommand{\adeval}[0]{{\mathcal{D}^\mathrm{ADE}_\mathrm{val}}}
\newcommand{\adetest}[0]{{\mathcal{D}^\mathrm{ADE}_\mathrm{test}}}
\newcommand{\adevalstar}[0]{{\mathcal{D}^\mathrm{ADE}_\mathrm{val*}}}
\newcommand{\adeteststar}[0]{{\mathcal{D}^\mathrm{ADE}_\mathrm{test*}}}
\newcommand{\adedev}[0]{{\mathcal{D}^\mathrm{ADE}_\mathrm{dev}}}

\newcommand{\bddtrain}[0]{{\mathcal{D}^\mathrm{BDD}_\mathrm{train}}}
\newcommand{\bddval}[0]{{\mathcal{D}^\mathrm{BDD}_\mathrm{val}}}
\newcommand{\bddtest}[0]{{\mathcal{D}^\mathrm{BDD}_\mathrm{test}}}
\newcommand{\bddvalstar}[0]{{\mathcal{D}^\mathrm{BDD}_\mathrm{val*}}}
\newcommand{\bddteststar}[0]{{\mathcal{D}^\mathrm{BDD}_\mathrm{test*}}}
\newcommand{\bdddev}[0]{{\mathcal{D}^\mathrm{BDD}_\mathrm{dev}}}

\newcommand{\mvtrain}[0]{{\mathcal{D}^\mathrm{MV}_\mathrm{train}}}
\newcommand{\mvval}[0]{{\mathcal{D}^\mathrm{MV}_\mathrm{val}}}
\newcommand{\mvtest}[0]{{\mathcal{D}^\mathrm{MV}_\mathrm{test}}}
\newcommand{\mvvalstar}[0]{{\mathcal{D}^\mathrm{MV}_\mathrm{val*}}}
\newcommand{\mvteststar}[0]{{\mathcal{D}^\mathrm{MV}_\mathrm{test*}}}
\newcommand{\mvdev}[0]{{\mathcal{D}^\mathrm{MV}_\mathrm{dev}}}

\newcommand{\acdctrain}[0]{{\mathcal{D}^\mathrm{ACDC}_\mathrm{train}}}
\newcommand{\acdcval}[0]{{\mathcal{D}^\mathrm{ACDC}_\mathrm{val}}}
\newcommand{\acdctest}[0]{{\mathcal{D}^\mathrm{ACDC}_\mathrm{test}}}
\newcommand{\acdcvalstar}[0]{{\mathcal{D}^\mathrm{ACDC}_\mathrm{val*}}}
\newcommand{\acdcteststar}[0]{{\mathcal{D}^\mathrm{ACDC}_\mathrm{test*}}}
\newcommand{\acdcdev}[0]{{\mathcal{D}^\mathrm{ACDC}_\mathrm{dev}}}

\newcommand{\kittitrain}[0]{{\mathcal{D}^\mathrm{KIT}_\mathrm{train}}}
\newcommand{\kittival}[0]{{\mathcal{D}^\mathrm{KIT}_\mathrm{val}}}
\newcommand{\kittitest}[0]{{\mathcal{D}^\mathrm{KIT}_\mathrm{test}}}
\newcommand{\kittivalstar}[0]{{\mathcal{D}^\mathrm{KIT}_\mathrm{val*}}}
\newcommand{\kittiteststar}[0]{{\mathcal{D}^\mathrm{KIT}_\mathrm{test*}}}
\newcommand{\kittidev}[0]{{\mathcal{D}^\mathrm{KIT}_\mathrm{dev}}}

\newcommand{\gtavfull}[0]{{\mathcal{D}^\mathrm{GTA5}_\mathrm{full}}}
\newcommand{\gtavtrain}[0]{{\mathcal{D}^\mathrm{GTA5}_\mathrm{train}}}
\newcommand{\gtavval}[0]{{\mathcal{D}^\mathrm{GTA5}_\mathrm{val}}}
\newcommand{\gtavtest}[0]{{\mathcal{D}^\mathrm{GTA5}_\mathrm{test}}}
\newcommand{\gtavvalstar}[0]{{\mathcal{D}^\mathrm{GTA5}_\mathrm{val*}}}
\newcommand{\gtavteststar}[0]{{\mathcal{D}^\mathrm{GTA5}_\mathrm{test*}}}
\newcommand{\gtavdev}[0]{{\mathcal{D}^\mathrm{GTA5}_\mathrm{dev}}}

\newcommand{\synthiafull}[0]{{\mathcal{D}^\mathrm{SYN}_\mathrm{full}}}
\newcommand{\synthiatrain}[0]{{\mathcal{D}^\mathrm{SYN}_\mathrm{train}}}
\newcommand{\synthiaval}[0]{{\mathcal{D}^\mathrm{SYN}_\mathrm{val}}}
\newcommand{\synthiatest}[0]{{\mathcal{D}^\mathrm{SYN}_\mathrm{test}}}
\newcommand{\synthiavalstar}[0]{{\mathcal{D}^\mathrm{SYN}_\mathrm{val*}}}
\newcommand{\synthiateststar}[0]{{\mathcal{D}^\mathrm{SYN}_\mathrm{test*}}}
\newcommand{\synthiadev}[0]{{\mathcal{D}^\mathrm{SYN}_\mathrm{dev}}}

\fi

==> tu_bs_colors.tex <==
\definecolor{tu0}{rgb}{0.7451, 0.1176, 0.2353}

\definecolor{tu1}{rgb}{1.0000, 0.8039, 0.0000}
\definecolor{tu11}{rgb}{1.0000, 0.8627, 0.3020}
\definecolor{tu12}{rgb}{1.0000, 0.9020, 0.4980}
\definecolor{tu13}{rgb}{1.0000, 0.9412, 0.6980}
\definecolor{tu14}{rgb}{1.0000, 0.9608, 0.8000}

\definecolor{tu2}{rgb}{0.9804, 0.4314, 0.0000}
\definecolor{tu21}{rgb}{0.9882, 0.6039, 0.3020}
\definecolor{tu22}{rgb}{0.9882, 0.7137, 0.4980}
\definecolor{tu23}{rgb}{0.9922, 0.8275, 0.6980}
\definecolor{tu24}{rgb}{0.9961, 0.8863, 0.8000}

\definecolor{tu3}{rgb}{0.6902, 0.0000, 0.2745}
\definecolor{tu31}{rgb}{0.7529, 0.2000, 0.4196}
\definecolor{tu32}{rgb}{0.8431, 0.4980, 0.6353}
\definecolor{tu33}{rgb}{0.9216, 0.7490, 0.8196}
\definecolor{tu34}{rgb}{0.9529, 0.8510, 0.8902}

\definecolor{tu4}{rgb}{0.4863, 0.8039, 0.9020}
\definecolor{tu41}{rgb}{0.6431, 0.8627, 0.9333}
\definecolor{tu42}{rgb}{0.7412, 0.9020, 0.9490}
\definecolor{tu43}{rgb}{0.8431, 0.9412, 0.9686}
\definecolor{tu44}{rgb}{0.8980, 0.9608, 0.9804}

\definecolor{tu5}{rgb}{0.0000, 0.5020, 0.7059}
\definecolor{tu51}{rgb}{0.3020, 0.6510, 0.7961}
\definecolor{tu52}{rgb}{0.5490, 0.7765, 0.8667}
\definecolor{tu53}{rgb}{0.7490, 0.8745, 0.9255}
\definecolor{tu54}{rgb}{0.8510, 0.9255, 0.9569}

\definecolor{tu6}{rgb}{0.0000, 0.3255, 0.4549}
\definecolor{tu61}{rgb}{0.2510, 0.4941, 0.5922}
\definecolor{tu62}{rgb}{0.5490, 0.6941, 0.7529}
\definecolor{tu63}{rgb}{0.7490, 0.8314, 0.8627}
\definecolor{tu64}{rgb}{0.8510, 0.8980, 0.9176}

\definecolor{tu7}{rgb}{0.0314, 0.0314, 0.0314}
\definecolor{tu71}{rgb}{0.3725, 0.3725, 0.3725}
\definecolor{tu72}{rgb}{0.5882, 0.5882, 0.5882}
\definecolor{tu73}{rgb}{0.7529, 0.7529, 0.7529}
\definecolor{tu74}{rgb}{0.8667, 0.8667, 0.8667}

\definecolor{tu8}{rgb}{0.7765, 0.9333, 0.0000}
\definecolor{tu81}{rgb}{0.8431, 0.9529, 0.3020}
\definecolor{tu82}{rgb}{0.8863, 0.9647, 0.4980}
\definecolor{tu83}{rgb}{0.9333, 0.9804, 0.6980}
\definecolor{tu84}{rgb}{0.9569, 0.9882, 0.8000}

\definecolor{tu9}{rgb}{0.5373, 0.6431, 0.0000}
\definecolor{tu91}{rgb}{0.6784, 0.7490, 0.3020}
\definecolor{tu92}{rgb}{0.7686, 0.8196, 0.4980}
\definecolor{tu93}{rgb}{0.8588, 0.8941, 0.6980}
\definecolor{tu94}{rgb}{0.9059, 0.9294, 0.8000}

\definecolor{tu10}{rgb}{0.0000, 0.4431, 0.3373}
\definecolor{tu101}{rgb}{0.3020, 0.6118, 0.5373}
\definecolor{tu102}{rgb}{0.5490, 0.7490, 0.7020}
\definecolor{tu103}{rgb}{0.7490, 0.8588, 0.8353}
\definecolor{tu104}{rgb}{0.8549, 0.9176, 0.9059}

\definecolor{tu110}{rgb}{0.8000, 0.0000, 0.6000}
\definecolor{tu111}{rgb}{0.8706, 0.3490, 0.7412}
\definecolor{tu112}{rgb}{0.9216, 0.6000, 0.8392}
\definecolor{tu113}{rgb}{0.9608, 0.8000, 0.9216}
\definecolor{tu114}{rgb}{0.9804, 0.8980, 0.9608}

\definecolor{tu120}{rgb}{0.4627, 0.0000, 0.4627}
\definecolor{tu121}{rgb}{0.5961, 0.2510, 0.5961}
\definecolor{tu122}{rgb}{0.7294, 0.4980, 0.7294}
\definecolor{tu123}{rgb}{0.8392, 0.6980, 0.8392}
\definecolor{tu124}{rgb}{0.9216, 0.8510, 0.9216}

\definecolor{tu130}{rgb}{0.4627, 0.0000, 0.3294}
\definecolor{tu131}{rgb}{0.6118, 0.3020, 0.5333}
\definecolor{tu132}{rgb}{0.7569, 0.5490, 0.6980}
\definecolor{tu133}{rgb}{0.8667, 0.7490, 0.8314}
\definecolor{tu134}{rgb}{0.9216, 0.8510, 0.9020}

\definecolor{GreenLight}{cmyk}{0.4,0.0,1.0,0.0}
\definecolor{Green}{cmyk}{0.45,0.0,1.0,0.4}
\definecolor{GreenDark}{cmyk}{0.94,0.0,0.59,0.64}
